Full-Duplex Massive MIMO Cellular Networks with Low Resolution ADC/DAC

In this paper, we provide an analytical framework for full-duplex (FD) massive multiple-input multiple-output (MIMO) cellular networks with low resolution analog-to-digital and digital-to-analog converters (ADCs and DACs). Matched filters are employed at the FD base stations (BSs) at the transmit and receive sides. For both reverse and forward links, our contributions are (1) derivations of the signal-to-quantization-plus-interference-and-noise ratio (SQINR) for general and special cases; (2) derivations of spectral efficiency for asymptotic cases as well as for power scaling laws; and (3) quantifying effects of quantization error, loopback self-interference, and inter-user interference for hexagonal cells and Poisson Point Process (PPP) tessellations on outage probability and spectral efficiency.

==> performance.tex <==
\section{Performance Analysis}
\begin{table}[H]
\renewcommand{\arraystretch}{1}
\caption{Power Consumption of Each Device \cite{adc}.}
\label{param}
\centering
\begin{tabular}{rll}
\bfseries Device & \bfseries Notation & \bfseries Value\\
\hline
Low Noise Amplifier (LNA) \cite{adc36} & $\rho_{\text{LNA}}$ & 39 mW\\
Splitter & $\rho_{\text{SP}}$ & 19.5 mW\\
Combiner \cite{adc36} & $\rho_{\text{C}}$ & 19.5 mW\\
Phase Shifter \cite{adc37,adc38} & $\rho_{\text{PS}}$ & 2 mW\\
Mixer \cite{adc39} & $\rho_{\text{M}}$  & 16.8 mW\\
Local Oscillator \cite{adc27} & $\rho_{\text{LO}}$ & 5 mW\\
Low Pass Filter \cite{adc27} & $\rho_{\text{LPF}}$ & 14 mW\\
Baseband Amplifier \cite{adc27} & $\rho_{\text{B}\text{B}_{\text{amp}} }$ & 5 mW\\
ADC & $\rho_{\text{ADC}}$ & $cB2^b$
\end{tabular}
\end{table}


\begin{table}[H]
\renewcommand{\arraystretch}{1}
\caption{ADC Power Consumption Per Sample Per Level, $c$ \cite{adc}.}
\label{param}
\centering
\begin{tabular}{rll}
\bfseries Scenario & \bfseries Value & \bfseries Generation\\
\hline
LPADC & 5 fJ/step/Hz & Ideal future value\\
IPADC & 65 fJ/step/Hz & Intermediate Power\\
HPADC & 494 fJ/step/Hz & State of the art\\
\end{tabular}
\end{table}

